7DGS: Unified Spatial-Temporal-Angular Gaussian Splatting

Real-time rendering of dynamic scenes with view-dependent effects remains a fundamental challenge in computer graphics. While recent advances in Gaussian Splatting have shown promising results separately handling dynamic scenes (4DGS) and view-dependent effects (6DGS), no existing method unifies these capabilities while maintaining real-time performance. We present 7D Gaussian Splatting (7DGS), a unified framework representing scene elements as seven-dimensional Gaussians spanning position (3D), time (1D), and viewing direction (3D). Our key contribution is an efficient conditional slicing mechanism that transforms 7D Gaussians into view- and time-conditioned 3D Gaussians, maintaining compatibility with existing 3D Gaussian Splatting pipelines while enabling joint optimization. Experiments demonstrate that 7DGS outperforms prior methods by up to 7.36 dB in PSNR while achieving real-time rendering (401 FPS) on challenging dynamic scenes with complex view-dependent effects. The project page is: https://gaozhongpai.github.io/7dgs/.

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------



==> sec/2_method.tex <==
\section{Method}

\subsection{7D Gaussian Representation}

We represent a dynamic scene as a collection of 7D Gaussians. Each Gaussian $G_i$ is parameterized by:

\begin{equation}
G_i = (\bm{\mu}_i, \bm{\Sigma}_i, \alpha_i, \bm{\beta}_i(t))
\end{equation}

where:
\begin{itemize}
    \item $\bm{\mu}_i \in \mathbb{R}^7$ is the mean in the joint space
    \item $\bm{\Sigma}_i \in \mathbb{R}^{7\times7}$ is the covariance matrix
    \item $\alpha_i \in \mathbb{R}$ is the base opacity
    \item $\bm{\beta}_i(t) \in \mathbb{R}^{48}$ are time-varying spherical harmonics coefficients
\end{itemize}

The joint distribution can be written in block form:

\begin{equation}
\begin{bmatrix} 
\mathbf{X}_p \\ 
\mathbf{X}_t \\ 
\mathbf{X}_d 
\end{bmatrix} \sim 
\mathcal{N}\left(
\begin{bmatrix} 
\bm{\mu}_p \\ 
\mu_t \\ 
\bm{\mu}_d
\end{bmatrix},
\begin{bmatrix} 
\bm{\Sigma}_{pp} & \bm{\Sigma}_{pt} & \bm{\Sigma}_{pd} \\
\bm{\Sigma}_{tp} & \sigma_{tt} & \bm{\Sigma}_{td} \\
\bm{\Sigma}_{dp} & \bm{\Sigma}_{dt} & \bm{\Sigma}_{dd}
\end{bmatrix}
\right)
\end{equation}

\subsection{Two-Stage Conditional Slicing}
For efficient rendering, we introduce a novel two-stage conditional slicing approach that first conditions on time and then on viewing direction:

\subsubsection{Stage 1: Temporal Conditioning}
First, we compute the distribution conditioned on time:

\begin{equation}
p(\mathbf{X}_p, \mathbf{X}_d|\mathbf{X}_t=t) = \mathcal{N}(\bm{\mu}_t, \bm{\Sigma}_t)
\end{equation}

where:
\begin{equation}
\bm{\mu}_t = \begin{bmatrix}
\bm{\mu}_p + \bm{\Sigma}_{pt}\sigma_{tt}^{-1}(t-\mu_t) \\
\bm{\mu}_d + \bm{\Sigma}_{dt}\sigma_{tt}^{-1}(t-\mu_t)
\end{bmatrix}
\end{equation}

\begin{equation}
\bm{\Sigma}_t = \begin{bmatrix}
\bm{\Sigma}_{pp} - \bm{\Sigma}_{pt}\sigma_{tt}^{-1}\bm{\Sigma}_{tp} & 
\bm{\Sigma}_{pd} - \bm{\Sigma}_{pt}\sigma_{tt}^{-1}\bm{\Sigma}_{td} \\
\bm{\Sigma}_{dp} - \bm{\Sigma}_{dt}\sigma_{tt}^{-1}\bm{\Sigma}_{tp} & 
\bm{\Sigma}_{dd} - \bm{\Sigma}_{dt}\sigma_{tt}^{-1}\bm{\Sigma}_{td}
\end{bmatrix}
\end{equation}

\subsubsection{Stage 2: Directional Conditioning}
Next, we condition on the viewing direction:

\begin{equation}
p(\mathbf{X}_p|\mathbf{X}_d=\mathbf{d}, \mathbf{X}_t=t) = \mathcal{N}(\bm{\mu}_\text{cond}, \bm{\Sigma}_\text{cond})
\end{equation}

where:
\begin{equation}
\bm{\mu}_\text{cond} = \bm{\mu}_{p|t} + \bm{\Sigma}_{pd|t}\bm{\Sigma}_{dd|t}^{-1}(\mathbf{d}-\bm{\mu}_{d|t})
\end{equation}

\begin{equation}
\bm{\Sigma}_\text{cond} = \bm{\Sigma}_{pp|t} - \bm{\Sigma}_{pd|t}\bm{\Sigma}_{dd|t}^{-1}\bm{\Sigma}_{pd|t}^\top
\end{equation}

This two-stage approach offers several advantages:
\begin{itemize}
    \item Reduced computational complexity
    \item Better numerical stability
    \item Clearer physical interpretation
    \item Easier optimization
\end{itemize}

\subsection{View and Time-Dependent Opacity}

The opacity is modulated by both temporal and directional factors through carefully designed modulation functions:

\begin{equation}
f_\text{cond}^t = \exp(-\lambda_t(t - \mu_t)^\top\sigma_{tt}^{-1}(t - \mu_t))
\end{equation}

\begin{equation}
f_\text{cond}^d = \exp(-\lambda_d(\mathbf{d} - \bm{\mu}_d)^\top\bm{\Sigma}_{dd}^{-1}(\mathbf{d} - \bm{\mu}_d))
\end{equation}

The final conditional opacity is:

\begin{equation}
\alpha_\text{cond} = \alpha \cdot \sqrt{f_\text{cond}^t \cdot f_\text{cond}^d}
\end{equation}

The parameters $\lambda_t$ and $\lambda_d$ control the strength of temporal and directional modulation respectively. We explore both fixed and learnable versions of these parameters.

\subsection{Time-Varying View-Dependent Color}

We extend traditional spherical harmonics to incorporate temporal variation:

\begin{equation}
c(\mathbf{d},t) = \text{sigmoid}\left(\sum_{\ell=0}^L \sum_{m=-\ell}^\ell \beta_{\ell m}(t)Y_{\ell m}(\mathbf{d})\right)
\end{equation}

The time-varying coefficients are modeled using a Fourier basis:

\begin{equation}
\beta_{\ell m}(t) = \sum_{n=0}^N w_{\ell m n}\cos\left(\frac{2\pi nt}{T}\right)
\end{equation}

This formulation enables:
\begin{itemize}
    \item Efficient computation
    \item Smooth temporal variation
    \item Compact representation
    \item Easy optimization
\end{itemize}


==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
